Eigenvalue Results for Large Scale Random Vandermonde Matrices with Unit Complex Entries

This paper centers on the limit eigenvalue distribution for random Vandermonde matrices with unit magnitude complex entries. The phases of the entries are chosen independently and identically distributed from the interval $[-\pi,\pi]$. Various types of distribution for the phase are considered and we establish the existence of the empirical eigenvalue distribution in the large matrix limit on a wide range of cases. The rate of growth of the maximum eigenvalue is examined and shown to be no greater than $O(\log N)$ and no slower than $O(\log N/\log\log N)$ where $N$ is the dimension of the matrix. Additional results include the existence of the capacity of the Vandermonde channel (limit integral for the expected log determinant).

==> indpnteqns.tex <==

\subsection{Random Vandermonde Matrices}
\vspace{0.3cm}
We now show that there is a real symmetric matrix which has the
same eigenvalues as ${\bf V^{*}V}$ where ${\bf V}$ is the random Vandermonde matrix.
\vspace{0.3cm}
\begin{lemma}
\label{lemma_equiv}
Let ${\bf A}, {\bf B}\in\cmplx^{N \times N}$ and suppose that
\begin{equation}
\label{eqn_component}
B_{k,\ell} = \frac{c_k}{c_\ell} A_{k,\ell}
\end{equation}
with $c_k \neq 0$ and $k=1,\cdots,N$. Then ${\bf A,B}$ have the same eigenvalues.
\end{lemma}

\vspace{0.3cm}
\noindent The proof of this result can be found in the appendix. 

\vspace{0.3cm}
\begin{cor} \label{corr_complexreal}
The matrix ${\bf X_{N}}$ with entries
$$
X_{i,j} = \Bigg( \frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}\Bigg)
$$
has the same eigenvalues as ${\bf V^{*}V}$
\end{cor}
\vspace{0.3cm}
\noindent The proof of this result can be found in the appendix. 

\subsection{Random Vandermonde Coefficients}
Let $\rho\in\mathcal{P}(n)$  be a partition of the set $\{1,2,\ldots,n\}$ and let $\{M_{1},M_{2},\ldots,M_{n}\}$ be variables with $0\leq M_{k}\leq 1$. For each block of the partition $\rho$ we consider the corresponding block partition equation as they were defined in \cite{GC02} and \cite{SP}. It is clear that when we consider all the $B$ equations we have $n+1-B$ free variables. It was proved in \cite{GC02} that the Vandermonde expansion coefficient $K_{\rho,u}$ associated with the uniform distribution is given by
$$
K_{\rho,u}=\text{volume of the solution set in $[0,1]^{n+1-B}$}
$$
which is the volume of the associated polytope. Consider the map $\rho:\{1,2,\ldots,n\}\to\{1,2,\ldots,B\}$ such that $\rho(i)=k$ if and only if $i$ is in block $k$. The analysis done in \cite{GC02} and \cite{SP} with respect to these coefficients can be summarized as
\begin{equation}
 K_{\rho,u}=\lim_{N}{K_{\rho,u,N}}
\end{equation}
where 
\begin{eqnarray}
K_{\rho,u,N} & = & \frac{1}{N^{n+1}}\cdot\frac{N!}{(2\pi)^{B}(N-B)!}\cdot \\
& \cdot & \int_{[-\pi,\pi]^{B}}{F_{\rho}(x_{1},\ldots,x_{B})\,dx_{1}\ldots dx_{B}} \nonumber 
\end{eqnarray}
with 
$$
F_{\rho}(x_{1},\ldots,x_{B}):=\prod_{j=1}^{n}{F(x_{\rho(j)}-x_{\rho(j+1)})}
$$
and
$$F(x)=\frac{\sin(\frac{N}{2}x)}{\sin(\frac{x}{2})}.$$


==> max_eig_ub_rev.tex <==
Let ${\bf V}$ be a square $N\times N$ random Vandermonde matrix with phase distribution $\nu$. In this Section we will focus on the study of growth of the maximum eigenvalue of the matrix ${\bf V^{*}V}$ as a function of $N$. More specifically, we know that the matrix ${\bf V^{*}V}$ is a positive definite $N\times N$ random matrix with eigenvalues $\{\lambda_{1}\leq\lambda_{2}\leq\ldots\leq\lambda_{N}\}$. It is clear that $\lambda_{N}$ is a random variable with values in the interval $[0,N]$. The value $N$ is taken by the random variable $\lambda_{N}$ in the event in which all the phases in the random matrix are equal ($\theta_{1}=\theta_{2}=\ldots=\theta_{N}$) and this event has zero probability. First we will prove an upper bound on the expectation $\mathbb{E}[\lambda_{N}]$.

\vspace{0.2cm}

\noindent Note that, of course, such a study does not rely on the existence of a limiting measure. 

\subsection{Upper bound}
\label{max_upper}

We first note that the matrix ${\bf V^{*}V}$ has the same eigenvalues as the matrix 
$$
{\bf X}_{N}=\Bigg( \frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}\Bigg)_{1\leq i,j\leq N}.
$$
See Appendix A for a proof of this statement. It is a well known result in Linear Algebra (see \cite{Horn}) that 
$$
\lambda_{N}\leq (\max_{i}\{c_{i}\}\max_{i}\{r_{i}\})^{\frac{1}{2}}
$$ 
where 
$c_i$ and $r_i$ are the $l_{1}$ norms of the columns and rows of the matrix. In this particular case,
$$
r_{i}:=\sum_{j=1}^{N}{\babs{\frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}}}
$$ 
and 
$$c_{i}:=\sum_{j=1}^{N}{\babs{\frac{\sin(\frac{N}{2}(\theta_{j}-\theta_{i}))}{N\sin(\frac{\theta_{j}-\theta_{i}}{2})}}}.
$$ 
Therefore, in this cases $r_i = c_i$ and the maximum eigenvalue $\lambda_{N}$ satisfies 
$$
\lambda_{N}\leq\max\{ r_{i}\,:\,i=1,2,\ldots,N\}.
$$ 
Each $r_{i}$ is a random variable with distribution 
$$
Y=1+X_{1}+X_{2}+\ldots+X_{N-1}
$$ 
where $X_{1},\ldots, X_{N-1}$ are independent identically distributed random variables with the same distribution as 
$$
X(\theta):=\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}\hspace{0.1cm}\text{where $\theta$ is distributed accordingly to $\nu$}.
$$

\noindent We will assume that $\nu$ is a probability measure on $[-\pi,\pi]$ which is absolutely continuous with respect to Lebesgue measure and with bounded pdf $f\in L^{\infty}([-\pi,\pi])$. 

\vspace{0.3cm}
\begin{remark}
The random variable $X(\theta)$ has expectation 
$$\mathbb{E}(X(\theta))=\int_{-\pi}^{\pi}{\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}f(\theta)\,d\theta}$$

\noindent and second moment 
$$\mathbb{E}(X(\theta)^{2})=\int_{-\pi}^{\pi}{\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}^{2}f(\theta)\,d\theta}.$$

\noindent In case $\nu$ is the uniform distribution then $f(\theta)=\frac{1}{2\pi}$ and using the results on the integral of the Dirichlet kernel (see \cite{Dirichlet}) we see that: 
$$\mathbb{E}(X(\theta))\asymp \frac{\log N}{N}.$$

\noindent Using Parseval's Theorem it is straightforward to see that $$\mathbb{E}(X(\theta)^{2})=\frac{1}{N}.$$
\end{remark}

\vspace{0.3cm}

\begin{theorem}\label{upper_teo}
For every $\epsilon>0$ and every $u\geq 0$ we have that 
\begin{equation}
\mathbb{P}\Big(\lambda_{N}\geq (C+\epsilon)\log N +u\Big)\leq K\frac{e^{-u}}{N^{\epsilon}}
\end{equation}

\noindent where $K>0$ is a constant independent on $\epsilon, u$ and $N$ and $C=\big(4\pi\norm{f}_{\infty}(e-1)+1\big)$.
\end{theorem}

\vspace{0.2cm}
\noindent Note that for $\epsilon = 1+\delta, \delta >0$ the result implies that 
$\lambda_N > (C+\epsilon)\log N$ occurs finitely many times a.s. by the First Borel-Cantelli lemma. 

\vspace{0.2cm}
\noindent As a Corollary we have:
\vspace{0.3cm}

\begin{cor}
 \begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + o(1).
\end{equation}
\end{cor}

\noindent We will first prove Theorem \ref{upper_teo}. 

\vspace{0.2cm}
\begin{proof}
It is easy to see that
\begin{equation}\label{eq_char} 
\babs{\frac{\sin(\frac{N}{2}\abs{x})}{N\sin(\frac{\abs{x}}{2})}}\leq\sum_{k=1}^{N/2}{\,\frac{1}{k}\cdot\,\mathbf{1}_{[\frac{2\pi(k-1)}{N},\frac{2\pi k}{N})}(\abs{x})}
\end{equation}

\noindent for every $x\in [-\pi,\pi]$. Let us define $p_{k}=\nu([\frac{2\pi(k-1)}{N},\frac{2\pi k}{N}])$ and $p_{-k}:=\nu([-\frac{2\pi k}{N},-\frac{2\pi(k-1)}{N}])$ and let $q_{k}=p_{k}+p_{-k}$ for every $k=1,2,\ldots, \frac{N}{2}$.

\noindent Hence, for every $t\in [0,1]$
$$\mathbb{E}(e^{Xt})\leq \sum_{k=1}^{N/2}{q_{k}e^{\frac{t}{k}}}\leq 1+(e-1)\sum_{k=1}^{N/2}{q_{k}\frac{t}{k}}$$

\noindent where the first inequality comes from (\ref{eq_char}) and the last inequality comes from the fact that $e^{t}\leq 1+(e-1)t$ for every $t\in [0,1]$. Since $\max_{k}\{p_{k},p_{-k}\}\leq \frac{2\pi}{N}\norm{f}_{\infty}$ we conclude that 
$$
\mathbb{E}(e^{X})\leq 1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2}
$$
\noindent where $H_{p}:=\sum_{k=1}^{p}{\frac{1}{k}}$ is the Harmonic series.

\vspace{0.2cm}
The random variables $r_{i}$ have the same distribution as
$$
Y=1+X_{1}+\ldots+X_{N-1}
$$ 
where $\{X_{1},\ldots,X_{N-1}\}$ are i.i.d. as
$X$. However, they are not independent. Using the Chernoff bound with the random variable $Y$ and $t=1$ (see \cite{Feller_Vol1}) we see that:
\begin{eqnarray*}
\mathbb{P}\Big(Y &\geq & C\log(N)+u \Big) \leq  \mathbb{E}(e^{X})^{N}\cdot e^{-(C\log N + u)}\\
   &\leq &\frac{e^{-u}}{N^{C}}\cdot\Bigg( 1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2} \Bigg)^{N}.
\end{eqnarray*}

\noindent For any positive function $f:\mathbb{N}\to [0,+\infty)$ 
\begin{eqnarray*}
\Bigg( 1+\frac{f(N)}{N}\Bigg)^{N} & = & \mathrm{exp}\Bigg[ N\log\Bigg(1+\frac{f(N)}{N}\Bigg)\Bigg] \\
 & \leq & \mathrm{exp}(f(N))
\end{eqnarray*}

\noindent where the last inequality comes from the fact that $\log(1+x)\leq x$ for all $x\geq 0$. 

\vspace{0.3cm}
\noindent Hence, 
\begin{equation*}
\Bigg(1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2} \Bigg)^{N} \leq\mathrm{exp}\Bigg[ 4\pi\norm{f}_{\infty}H_{N/2}\Bigg]
\end{equation*}

\noindent and since $H_{p}\leq\log{p}+\gamma+\half p^{-1}$ where $\gamma$ is the Euler--Mascheroni constant $\gamma\approx 0.57721566...$ 
\begin{equation*}
 \mathrm{exp}\Bigg[ 4\pi\norm{f}_{\infty}H_{N/2}\Bigg]\leq K\cdot \mathrm{exp}\Bigg[ 4\pi\norm{f}_{\infty}(e-1) \log(N/2) \Bigg]
\end{equation*}

\noindent where $K=\mathrm{exp}(4\pi\norm{f}_{\infty}(e-1)\gamma)$.

\noindent Let us define the random variable $Z$ as $Z=\max_{k}\{r_{k}\}$. Therefore, 
\begin{eqnarray*}
\mathbb{P}(\lambda_{N}\geq C\log N+u) & \leq & \mathbb{P}(Z\geq C\log N+u)\\
  & \leq & N\mathbb{P}(Y\geq C\log N+u)
\end{eqnarray*}

\noindent where the last inequality comes from the union bound. Hence, for all $u\geq 0$ we have 
\begin{eqnarray*}
\mathbb{P}(\lambda_{N}\geq C\log N+u) & \leq & \frac{N}{N^{C}}Ke^{-u}\Bigg( \frac{N}{2}\Bigg)^{4\pi\norm{f}_{\infty}(e-1)} \\
  & \leq & K_{2}e^{-u}N^{(4\pi\norm{f}_{\infty}(e-1)+1-C)}.
\end{eqnarray*}

Let $\epsilon>0$ and let $C=4\pi\norm{f}_{\infty}(e-1)+1$. Then for every $u\geq 0$
$$\mathbb{P}(\lambda_{N}\geq (C+\epsilon)\log N +u)\leq K_{2}\frac{e^{-u}}{N^{\epsilon}}.$$
\end{proof}

\noindent Now we follow with the proof of the Corollary.

\vspace{0.2cm}

\begin{proof} Using the previous Theorem we have that,
\begin{eqnarray*}
\mathbb{E}(\lambda_{N}) & = & \int_{0}^{+\infty}{\mathbb{P}(\lambda_{N}\geq t)\,dt} \leq \int_{0}^{C\log N}{\mathbb{P}(\lambda_{N}\geq t)\,dt} \\
& + & \int_{0}^{+\infty}{\mathbb{P}(\lambda_{N}\geq C\log N+u)\,du} \\
& \leq & \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + \frac{K_{2}}{N^{\epsilon}}.
\end{eqnarray*}

\noindent Since $K_{2}$ does not depend on $N$ and $\epsilon$ is arbitrary we conclude that for $N$ sufficiently large 
\begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + o(1).
\end{equation}

\end{proof}

\begin{remark}
For the case $\nu$ is uniform distribution on $[-\pi,\pi]$ we have that 
\begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(2e-1\Big)\log N + o(1).
\end{equation}
\end{remark}

\begin{remark}
We believe that the constant $C$ in Theorem \ref{upper_teo} can be sharpened by working with the optimal choice for $t$.
\end{remark}


==> max_eig_ub_revjul21.tex <==
Let ${\bf V}$ be a square $N\times N$ random Vandermonde matrix with phase distribution $\nu$. In this Section we will focus on the study of growth of the maximum eigenvalue of the matrix ${\bf V^{*}V}$ as a function of $N$. More specifically, we know that the matrix ${\bf V^{*}V}$ is a positive definite $N\times N$ random matrix with eigenvalues $\{\lambda_{1}\leq\lambda_{2}\leq\ldots\leq\lambda_{N}\}$. It is clear that $\lambda_{N}$ is a random variable with values in the interval $[0,N]$. The value $N$ is taken by the random variable $\lambda_{N}$ in the event in which all the phases in the random matrix are equal ($\theta_{1}=\theta_{2}=\ldots=\theta_{N}$) and this event has zero probability. First we will prove an upper bound on the expectation $\mathbb{E}[\lambda_{N}]$.

\vspace{0.2cm}

\noindent Note that, of course, such a study does not rely on the existence of a limiting measure. 

\subsection{Upper bound}
\label{max_upper}

We first note that the matrix ${\bf V^{*}V}$ has the same eigenvalues as the matrix 
$$
{\bf X}_{N}=\Bigg( \frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}\Bigg)_{1\leq i,j\leq N}.
$$
See Appendix A for a proof of this statement. It is a well known result in Linear Algebra (see \cite{Horn}) that 
$$
\lambda_{N}\leq (\max_{i}\{c_{i}\}\max_{i}\{r_{i}\})^{\frac{1}{2}}
$$ 
where 
$c_i$ and $r_i$ are the $l_{1}$ norms of the columns and rows of the matrix. In this particular case,
$$
r_{i}:=\sum_{j=1}^{N}{\babs{\frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}}}
$$ 
and 
$$c_{i}:=\sum_{j=1}^{N}{\babs{\frac{\sin(\frac{N}{2}(\theta_{j}-\theta_{i}))}{N\sin(\frac{\theta_{j}-\theta_{i}}{2})}}}.
$$ 
Therefore, it is the case that $r_i = c_i$ and the maximum eigenvalue $\lambda_{N}$ satisfies 
$$
\lambda_{N}\leq\max\{ r_{i}\,:\,i=1,2,\ldots,N\}.
$$ 
Each $r_{i}$ is a random variable with distribution 
$$
Y=1+X_{1}+X_{2}+\ldots+X_{N-1}
$$ 
where $X_{1},\ldots, X_{N-1}$ are independent identically distributed random variables with the same distribution as 
$$
X(\theta):=\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}\hspace{0.1cm}\text{where $\theta$ is distributed accordingly to $\nu$}.
$$
save that we condition on the centering constant $\theta_i$. 
\noindent We will assume that $\nu$ is a probability measure on $[-\pi,\pi]$ which is absolutely continuous with respect to Lebesgue measure and with bounded pdf $f\in L^{\infty}([-\pi,\pi])$. In what follows the Chernoff bound construction will only make 
use of $\norm{f}_{\infty}$ and hence is independent of $\theta_i$.

\vspace{0.3cm}
\begin{remark}
The random variable $X(\theta)$ has expectation 
$$\mathbb{E}(X(\theta))=\int_{-\pi}^{\pi}{\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}f(\theta)\,d\theta}$$

\noindent and second moment 
$$\mathbb{E}(X(\theta)^{2})=\int_{-\pi}^{\pi}{\babs{\frac{\sin(\frac{N}{2}\theta)}{N\sin(\frac{\theta}{2})}}^{2}f(\theta)\,d\theta}.$$

\noindent In case $\nu$ is the uniform distribution then $f(\theta)=\frac{1}{2\pi}$ and using the results on the integral of the Dirichlet kernel (see \cite{Dirichlet}) we see that: 
$$\mathbb{E}(X(\theta))\asymp \frac{\log N}{N}.$$

\noindent Using Parseval's Theorem it is straightforward to see that $$\mathbb{E}(X(\theta)^{2})=\frac{1}{N}.$$
\end{remark}

\vspace{0.3cm}

\begin{theorem}\label{upper_teo}
Given $\epsilon>0$ and $\kappa in (0,1)$, then for every $u\geq 0$, $\exists N_{\kappa\epsilon}$ such that
$\forall N > N_{\kappa\epsilon}$,
\begin{equation}
\mathbb{P}\Big(\lambda_{N}\geq (C+\epsilon)\log N +u\Big)\leq K\frac{e^{-u}}{N^{\epsilon\kappa}}
\end{equation}

\noindent where $K>0$ is a constant independent on $\epsilon, u$ and $N$ and $C=\big(4\pi\norm{f}_{\infty}(e-1)+1\big)$.
\end{theorem}

\vspace{0.2cm}
\noindent Note that for $\epsilon = 1+\delta, \delta >0$ the result implies that 
$\lambda_N > (C+\epsilon)\log N$ occurs finitely many times a.s. by the First Borel-Cantelli lemma. 

\vspace{0.2cm}
\noindent As a Corollary we have:
\vspace{0.3cm}

\begin{cor}
 \begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + o(1).
\end{equation}
\end{cor}

\noindent We will first prove Theorem \ref{upper_teo}. 

\vspace{0.2cm}
\begin{proof}
It is easy to see that
\begin{equation}\label{eq_char} 
\babs{\frac{\sin(\frac{N}{2}\abs{x})}{N\sin(\frac{\abs{x}}{2})}}\leq\sum_{k=1}^{N/2}{\,\frac{1}{k}\cdot\,\mathbf{1}_{[\frac{2\pi(k-1)}{N},\frac{2\pi k}{N})}(\abs{x})}
\end{equation}

\noindent for every $x\in [-\pi,\pi]$. Let us define $p_{k}=\nu([\frac{2\pi(k-1)}{N},\frac{2\pi k}{N}])$ and $p_{-k}:=\nu([-\frac{2\pi k}{N},-\frac{2\pi(k-1)}{N}])$ and let $q_{k}=p_{k}+p_{-k}$ for every $k=1,2,\ldots, \frac{N}{2}$.

\noindent Hence, for every $t\in [0,1]$
$$\mathbb{E}(e^{Xt}|\theta_i)\leq \sum_{k=1}^{N/2}{q_{k}e^{\frac{t}{k}}}\leq 1+(e-1)\sum_{k=1}^{N/2}{q_{k}\frac{t}{k}}$$

\noindent where the first inequality comes from (\ref{eq_char}) and the last inequality comes from the fact that $e^{t}\leq 1+(e-1)t$ for every $t\in [0,1]$. Since $\max_{k}\{p_{k},p_{-k}\}\leq \frac{2\pi}{N}\norm{f}_{\infty}$ we conclude that 
\begin{equation}
\mathbb{E}(e^{X}|\theta_i)\leq 1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2}
\label{eqn_condlmom}
\end{equation}
\noindent where $H_{p}:=\sum_{k=1}^{p}{\frac{1}{k}}$ is the Harmonic series.

\vspace{0.2cm}
The random variables $r_{i}$ all have the same 
distribution as
$$
Y=1+X_{1}+\ldots+X_{N-1}
$$ 
where $\{X_{1},\ldots,X_{N-1}\}$ are i.i.d, conditional on $\theta_i$. % as %$X$. 
However, the $r_i$ are not independent. Using the Chernoff bound with the 
random variable $Y$, unconditioning and setting $t=1$ (see \cite{Feller_Vol1}) 
we see that:
\begin{eqnarray*}
\mathbb{P}\Big(Y &\geq & C\log(N)+u | \theta_i\Big) \leq  \mathbb{E}(e^{X}|\theta_i)^{N}\cdot 
e^{-(C_\delta\log N + u)}\\
   &\leq &\frac{e^{-u}}{N^{C_\delta}}\cdot\Bigg( 1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2} \Bigg)^{N}.
\end{eqnarray*}
This follows from the bound on the conditional mgf, (\ref{eqn_condlmom}). 
Here $C_\delta = C - \delta$ and $\delta >0$ satisfies $\delta \log N_\delta < 1$ so that the inequality holds
$\forall N \geq N_\delta$. Unconditioning,
$$
\mathbb{P}\Big(Y \geq  C\log(N)+u | \Big) \leq \frac{e^{-u}}{N^{C_\delta}}\cdot\Bigg( 1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2} \Bigg)^{N}.
$$

%\noindent 
For any positive function $f:\mathbb{N}\to [0,+\infty)$ 
\begin{eqnarray*}
\Bigg( 1+\frac{f(N)}{N}\Bigg)^{N} & = & \mathrm{exp}\Bigg[ N\log\Bigg(1+\frac{f(N)}{N}\Bigg)\Bigg] \\
 & \leq & \mathrm{exp}(f(N))
\end{eqnarray*}

\noindent where the last inequality comes from the fact that $\log(1+x)\leq x$ for all $x\geq 0$. 

\vspace{0.3cm}
\noindent Hence, 
\begin{equation*}
\Bigg(1+\frac{4\pi(e-1)\norm{f}_{\infty}}{N}\cdot H_{N/2} \Bigg)^{N} \leq\mathrm{exp}\Bigg[ 4\pi(e-1)\norm{f}_{\infty}H_{N/2}\Bigg]
\end{equation*}

\noindent and since $H_{p}\leq\log{p}+\gamma+\half p^{-1}$ where $\gamma$ is the Euler--Mascheroni constant $\gamma\approx 0.57721566...$ 
\begin{equation*}
 \mathrm{exp}\Bigg[ 4\pi(e-1)\norm{f}_{\infty}H_{N/2}\Bigg]\leq K\cdot \mathrm{exp}\Bigg[ 4\pi\norm{f}_{\infty}(e-1) \log(N/2) \Bigg]
\end{equation*}

\noindent where $K=\mathrm{exp}(4\pi\norm{f}_{\infty}(e-1)\gamma)$.

\noindent Let us define the random variable $Z$ as $Z=\max_{k}\{r_{k}\}$. Therefore, 
\begin{eqnarray*}
\mathbb{P}(\lambda_{N}\geq C\log N+u) & \leq & \mathbb{P}(Z\geq C\log N+u)\\
  & \leq & N\mathbb{P}(Y\geq C\log N+u)
\end{eqnarray*}

\noindent where the last inequality comes from the union bound. Hence, for all $u\geq 0$ we have 
\begin{eqnarray*}
\mathbb{P}(\lambda_{N}\geq C\log N+u) & \leq & \frac{N}{N^{C_\delta}}Ke^{-u}\Bigg( \frac{N}{2}\Bigg)^{4\pi\norm{f}_{\infty}(e-1)} \\
  & \leq & K_{2}e^{-u}N^{(4\pi\norm{f}_{\infty}(e-1)+1-C_\delta)}.
\end{eqnarray*}

Let $\epsilon>0$ and  $\kappa \in (0,1)$ be given. Set $\delta = \epsilon(1-\kappa) > 0$ and set $C=4\pi\norm{f}_{\infty}(e-1)+1+\delta$ so that for every $u\geq 0$ and $N > N_{\kappa\epsilon}$
$$\mathbb{P}(\lambda_{N}\geq (C+\epsilon)\log N +u)\leq K_{2}\frac{e^{-u}}{N^{\epsilon\kappa}}.$$
\end{proof}

\noindent Now we follow with the proof of the Corollary.

\vspace{0.2cm}

\begin{proof} Using the previous Theorem we have that,
\begin{eqnarray*}
\mathbb{E}(\lambda_{N}) & = & \int_{0}^{+\infty}{\mathbb{P}(\lambda_{N}\geq t)\,dt} \leq \int_{0}^{C\log N}{\mathbb{P}(\lambda_{N}\geq t)\,dt} \\
& + & \int_{0}^{+\infty}{\mathbb{P}(\lambda_{N}\geq C\log N+u)\,du} \\
& \leq & \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + \frac{K_{2}}{N^{\epsilon/2}},
\end{eqnarray*}
for sufficiently large $N$.

\noindent Since $K_{2}$ does not depend on $N$ and $\epsilon$ is arbitrary we conclude that for $N$ sufficiently large 
\begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(4\pi\norm{f}_{\infty}(e-1)+1\Big)\log N + o(1).
\end{equation}

\end{proof}

\begin{remark}
For the case $\nu$ is uniform distribution on $[-\pi,\pi]$ we have that 
\begin{equation}
\mathbb{E}(\lambda_{N})\leq  \Big(2e-1\Big)\log N + o(1).
\end{equation}
\end{remark}

\begin{remark}
We believe that the constant $C$ in Theorem \ref{upper_teo} can be sharpened by working with the optimal choice for $t$.
\end{remark}


==> symm.tex <==
\subsection{Random Vandermonde Matrices}
\vspace{0.3cm}
We now show that there is a real symmetric matrix which has the
same eigenvalues as ${\bf V^{*}V}$ where ${\bf V}$ is the random Vandermonde matrix.
\vspace{0.3cm}
\begin{lemma}
\label{lemma_equiv}
Let ${\bf A}, {\bf B}\in\cmplx^{N \times N}$ and suppose that
\begin{equation}
\label{eqn_component}
B_{k,\ell} = \frac{c_k}{c_\ell} A_{k,\ell}
\end{equation}
with $c_k \neq 0$ and $k=1,\cdots,N$. Then ${\bf A,B}$ have the same eigenvalues.
\end{lemma}

\vspace{0.3cm}
\noindent The proof of this result can be found in the appendix. 

\vspace{0.3cm}
\begin{cor} \label{corr_complexreal}
The matrix ${\bf X_{N}}$ with entries
$$
X_{i,j} = \Bigg( \frac{\sin(\frac{N}{2}(\theta_{i}-\theta_{j}))}{N\sin(\frac{\theta_{i}-\theta_{j}}{2})}\Bigg)
$$
has the same eigenvalues as ${\bf V^{*}V}$
\end{cor}

\vspace{0.3cm}
\noindent The proof of this result can be found in the appendix. 



